Dynamic MTU : Technique to reduce packet drops in IPv6 network resulted due to smaller path mtu size

With an increase in the number of internet users and the need to secure internet traffic, the unreliable IPv4 protocol has been replaced by a more secure protocol, called IPv6 for Internet system. The IPv6 protocol does not allow intermediate routers to fragment the on-going IPv6 packet. Moreover, due to IP tunneling, some extra headers are added to the IPv6 packet, exceeding the packet size higher than the maximum transmission unit (MTU), resulting in increase in packet drops. One probable solution is to find the MTU of every link in advance using the Internet Control Message Protocol (ICMP) packets and accordingly fragment the packets at the source itself. However, most of the intermediate routers and the network firewalls do not allow ICMP packets to traverse through their network, resulting in network black holes, where we cannot know the MTU of some links in advance. This method tries to handle the packet drops in IPv6 network by proposing a DMTU scheme where we dynamically adjust the MTU of each link depending upon the original size of the IPv6 packet, thereby reducing the number of packet drops by a significant amount. Using mathematical and graphical analysis, our scheme proves to be much more efficient than the state-of-the-art PMTUD scheme. In this paper the method, mathematical and graphical representations are focusing solely in IPv6 Internet communication.

==> abstract.tex <==
% With an increase in the number of internet users and the need to secure
% internet traffic, the unreliable IPv4 protocol has been replaced by a more
% secure protocol, called IPv6 for Internet system. The IPv6 protocol does not allow intermediate
% routers to fragment the on-going IPv6 packet. Moreover, due to IP tunneling,
% some extra headers are added to the IPv6 packet, exceeding the packet size
% higher than the maximum transmission unit (MTU), resulting in increase in packet drops.
%  One probable solution is to find the MTU of every link in advance using the \textit{Internet Control Message Protocol} (ICMP) packets and accordingly fragment the packets at the source
% itself. However, most of the intermediate routers and the network firewalls do
% not allow ICMP packets to traverse through their network, resulting in network
% black holes, where we cannot know the MTU of some links in advance. In this paper, we present a method \textit{Dynamic MTU} (DMTU) scheme which tries to handle the packet drops in IPv6 network, where we dynamically adjust the MTU of each link depending upon the original
% size of the IPv6 packet, thereby reducing the number of packet drops by a
% significant amount. In the new proposed method we subsidized the use of ICMP packets and the large packets are processed on the fly, which we believe to enhance the throughput and latency of the network. The method works in two scenarios Parallel mode (Works with PMTUD) and Standalone mode. Where the later one have zero dependency on ICMP packets. The working of this method is divided into two phases pre-phase and post-phase for the optimisation of the algorithm. Further, we discuss the previous start-of-the-art algorithms and their limitation which give rise the need of a robust algorithm design and discuss in detail the different algorithms designs and presenting the basic architectural design of the proposed method as a basic foundation for the implementation in IPv6 network. 


With an increase in the number of internet users and the need to secure
internet traffic, the unreliable IPv4 protocol has been replaced by a more
secure protocol, called IPv6 for Internet system. The IPv6 protocol does not allow intermediate
routers to fragment the on-going IPv6 packet. Moreover, due to IP tunneling,
some extra headers are added to the IPv6 packet, exceeding the packet size
higher than the maximum transmission unit (MTU), resulting in increase in packet drops.
 One probable solution is to find the MTU of every link in advance
using the \textit{Internet Control Message Protocol} (ICMP) packets and accordingly fragment the packets at the source
itself. However, most of the intermediate routers and the network firewalls do
not allow ICMP packets to traverse through their network, resulting in network
black holes, where we cannot know the MTU of some links in advance. This method
tries to handle the packet drops in IPv6 network by proposing a DMTU scheme
where we dynamically adjust the MTU of each link depending upon the original
size of the IPv6 packet, thereby reducing the number of packet drops by a
significant amount. Using mathematical and graphical analysis, our scheme
proves to be much more efficient than the state-of-the-art PMTUD scheme. In this paper the method, mathematical and graphical representations are focusing solely in IPv6 Internet communication.

% Using mathematical and graphical analysis, our scheme
% proves to be much more efficient than the state-of-the-art PMTUD scheme. In this paper the method, mathematical and graphical representations are focusing solely in IPv6 Internet communication.
